Simulation of Electrospray Emission Processes for Highly Conductive Liquids

An electrohydrodynamic numerical model is used to explore the electrospray emission behavior of both moderate and high electrical conductivity liquids under electrospray conditions. The Volume-of-Fluid method, incorporating a leaky-dielectric model with a charge relaxation consideration, is used to conserve charge to accurately model cone-jet formation and droplet breakup. The model is validated against experiments and agrees well with both droplet diameters and charge-to-mass ratio of emitted progeny droplets. The model examines operating conditions such as flow rate and voltage, with fluid properties also considered, such as surface tension, electrical conductivity, and viscosity for both moderate and high conductivity. For high conductivity and surface tension, the results show that high charge concentration along with the meniscus and convex cone shape results in a higher charge-to-mass ratio of the emitted droplets while lower conductivity and surface tension tend towards concave cone shapes and lower charge-to-mass droplets. Recirculation flows inside the bulk liquid are investigated across a range of non-dimensional flow rates, and electric Reynolds numbers. For high conductivity liquid emission at the minimum stable flow rate, additional recirculation cells develop near the cone tip suggesting the onset of the axisymmetric instability.

==> new.tex <==
An Electrospray Extraction model \cite{huh2019numerical} is a finite-volume based ElectroHydroDynamic numerical model to understand the physics of a cone-jet and droplet formation of an electrospray thruster. Volume-of-Fluid method is incorporated in the model to track the interface of the liquid allowing to accurately calculate the total charge and the charge-to-mass ratio of the emitted droplet. The model is quantitatively validated in both the moderate ($\sigma_{moderate}=6.7\times10^{-6} S/m$) and the high electrical conductivity ($\sigma_{high}=2.3\times10^{-4} S/m$) fluid regimes. The droplet diameter and the total current of the model shows a good agreement with the experimental measurements \cite{tang,gamero} and the scaling law equations \cite{ganan}. The Gauss’s law and the charge conservation equation are solved along with the Navier-Stokes equation for flow field and charge distribution. Charge distribution at the cone-to-jet region is investigated at various operating conditions (flow rate, voltage) and fluid properties (surface tension, electrical conductivity, viscosity). The results present higher charge distribution with relatively shorter cone-to-jet length at the region allowing high charge-to-mass ratio of the emitted droplet. By incorporating leaky-dielectric model with the charge relaxation consideration($\frac{\partial\rho_e}{\partial t}+\bnabla\bcdot\sigma\boldsymbol{E} = 0$), where $\rho_e$ is charge density and \boldsymbol{E} is electric field, charge is well conserved in the droplets allowing accurate measurements of droplet charge-to-mass ratios. 
The ionic liquid, EMI-Im(1-ethyl-3-methylimidazolium bis(trifluoromethylsulfonyl)imide) has been used as a propellant for the LISA-Pathfinder mission and is considered as a prospective propellant for future space missions\cite{john}. To validate the result, simulation is performed for a solution of the EMI-Im, TBP(tributyl phosphate) ranging from  $6.7\times10^{-6} S/m$ to $2.3\times10^{-4} S/m$. Applied voltage between the emitter and the extractor is 1766 V and a liquid flow rate ranging from $4\times10^{-11}$ $m^{3}/s$ to $9.56\times10^{-11}$ $m^{3}/s$. The droplet diameters are calculated in the range of 7-13 $\mu$m and the current of 20-51 nA which is in reasonable agreement with the average size of 5 $\mu$m of diameter and 50 nA of the current in experimental results\cite{gamero}. The concavity of the liquid meniscus affects the length of the cone-to-jet region from the fact that the increasing surface tension results in a convex shape of the bulk meniscus followed by a shorter concave meniscus that allows higher charge accumulation at the concave region. With higher charge accumulation, the emitted droplets then tend to have a higher droplet charge-to-mass ratio with the shorter length of the cone-to-jet region.
Along with the charge distribution, the onset of the recirculation flow inside the fluid bulk is investigated with varying critical operating conditions and fluid properties. High tangential electrostatic forces near both the emitter tip and the cone-to-jet region results in the onset of several recirculation flows inside the bulk fluid. This recirculation flow grows with lower flow rate as shown in Figure 1, and  higher voltage, surface tension, electrical conductivity and subsides with higher viscosity. A new non-dimensional parameter(H number) is defined to observe the effect of the flow conditions and the fluid properties on the charge-to-mass ratio of the droplet. The onset of the recirculation flow due to the high tangential E-force is observed at above 0.06 of the H number. 

\begin{figure}[hbt!]
\centering
\includegraphics[width=.5\textwidth]{recirculation.png}
\caption{Onset of recirculation flows inside the fluid bulk in different flow rates}
\end{figure}


The Electrohydrodynamic flow behavior is defined by the comparison between the charge relaxation time scale $t_{E}=\epsilon/\sigma$, where $\epsilon$ is electrical permittivity and ${\sigma}$ is electrical conductivity and the hydrodynamic characteristic time $t_{H}=L^{3}/Q$, , where L is characteristic length scale and Q is the flow rate. In low conductivity, the electrical conductivity is in the order of $1\times10^{-9}$ where the speed of the fluid flow is comparable to that of the charge movement. The charge convection has non-negligible effect in the charge transport equation.\cite{javier,sengupta} In moderate and high conductivity, on the other hand, the charge relaxation time is smaller than the hydrodynamic time scale. The charge convection effect is negligible on the performance of the electrospray. Also, due to the intrinsic numerical diffusion caused by the additional convection term, the mass and charge loss increase with higher conductivity. Therefore, the resultant equation can be derived as above and is consistent with \cite{saville,herrada} who derived the same equation from the Electrokinetics point of view. Also, the Volume-of-Fluid(VOF) method is employed in the code for the two-phase flow simulations. To treat and discretize the two different phases, electrical conductivity, permittivity, density values of the cells are determined proportional to the volume fraction of the cell. While \cite{tomar} used an arithmetic averaging of the given properties, in this research, to effectively conserve the charge inside the droplet, we devised a new way of calculating the cell properties based on the liquid and vacuum properties. The novel VOF sub-model allows better resolution of small-sized droplets and accurate charge-to-mass ratio of highly conductive liquid. Comparison of different numerical approaches for the electric field and charge density distribution enables improved simulations in comparison to current experiments. The ability to accurately model the formation of cone-jets and droplets for electrospray thrusters provides valuable insight for understanding the thruster operating conditions and design choices that enable desirable performance and lifetime.

==> table.tex <==
\begin{table}
  \begin{center}
\def~{\hphantom{0}}
  \begin{tabular}{lccc}
      liquid & $\rho (kg/m^3)$ & $\sigma (S/m)$ & $\gamma (N/m)$ & $\epsilon (F/m)$ & $\mu (Pa S)$ \\
       Heptane & 684 & $6.26\times10^-7$ & 0.0186 & 1.91 & $4.28\times10^-4$\\
       TBPT & 976 & $2.3\times10^-4$ & 0.028 & 8.91 & $3.59\times10^-3$\\
    
  \end{tabular}
  \caption{Values of $kd$ at which trapped modes occur when $\rho(\theta)=a$}
  \label{tab:kd}
  \end{center}
\end{table}
